From Neural Activity to Computation: Biological Reservoirs for Pattern Recognition in Digit Classification

In this paper, we present a biologically grounded approach to reservoir computing (RC), in which a network of cultured biological neurons serves as the reservoir substrate. This system, referred to as biological reservoir computing (BRC), replaces artificial recurrent units with the spontaneous and evoked activity of living neurons. A multi-electrode array (MEA) enables simultaneous stimulation and readout across multiple sites: inputs are delivered through a subset of electrodes, while the remaining ones capture the resulting neural responses, mapping input patterns into a high-dimensional biological feature space. We evaluate the system through a case study on digit classification using a custom dataset. Input images are encoded and delivered to the biological reservoir via electrical stimulation, and the corresponding neural activity is used to train a simple linear classifier. To contextualize the performance of the biological system, we also include a comparison with a standard artificial reservoir trained on the same task. The results indicate that the biological reservoir can effectively support classification, highlighting its potential as a viable and interpretable computational substrate. We believe this work contributes to the broader effort of integrating biological principles into machine learning and aligns with the goals of human-inspired vision by exploring how living neural systems can inform the design of efficient and biologically plausible models.

==> sec/4_results.tex <==
\section{Results}

To evaluate the performance of the BRC system, it is first essential to determine the most informative time window for reading out the network's response to stimulation. For this purpose, we analyzed the classification accuracy across different stimulation sessions while systematically varying the duration $W$ of the post-stimulus time window used to extract neural activity.

\cref{fig:acc_var_w} shows the results obtained by aggregating data from $n = 9$ independent stimulation sessions performed across multiple days and biological replicates. A clear decreasing trend emerges, with the highest classification accuracy consistently observed when $W = 5\,\si{\milli\second}$. This suggests that the most informative response — in terms of discriminability among different stimuli — occurs within the first few milliseconds following stimulation.

This result is expected, as the initial segment of the neural response primarily reflects the immediate, first-order activation of neurons directly connected to the stimulated electrodes. In biological terms, a $5\,\si{\milli\second}$ window roughly corresponds to the timescale of a single synaptic transmission, capturing the direct postsynaptic potentials triggered by the stimulus. At these early latencies, the signal is minimally affected by recurrent processing, spontaneous activity, or noise propagation, making it highly specific to the input pattern.
As the time window $W$ increases beyond this point, the recorded activity becomes increasingly influenced by indirect responses, recurrent network dynamics, and spontaneous background activity. 

\begin{figure}[t]
\centerline{\includegraphics[width=1.0\linewidth]{images/ACC_var_w.pdf}}
    \caption{\textbf{Accuracy variation across different readout windows.} For each stimulation session (n=9), classification accuracy was computed using neural responses extracted from different post-stimulus time windows, ranging from $5$ to $50\,\si{\milli\second}$.  The plot reports the mean accuracy $\pm$ standard error of the mean (SEM). This analysis highlights how the temporal integration window influences the effectiveness of the reservoir readout.}
    \label{fig:acc_var_w}
\end{figure}

\begin{figure*}[t]
\centerline{\includegraphics[width=1.0\linewidth]{images/acc_per_cat_mean.png}}
\caption{
\textbf{Mean classification accuracy per input category for each biological replicate.} 
Each box displays the average classification accuracy for a given stimulus category, computed over multiple stimulation sessions for each single biological replicate (BR 1, BR 2, BR 3). Accuracies are calculated using 5-fold cross-validation within each session and then averaged across the three stimulation sessions (Day 1, Day 2, Day 3).
The last row in the heatmap displays the average classification accuracy per category computed over different realizations of the noise for the Artificial Reservoir (AR).}
\label{fig:mean_acc_per_category}
\end{figure*}

\begin{figure*}[t]
\centerline{\includegraphics[width=1.0\linewidth]{images/acc_per_cat_mean_clf_pretrain.png}}
\caption{\textbf{Mean classification accuracy per input category across days.} 
Each box represents the average classification accuracy for a specific stimulus category, computed by training the classifier on data from Day 1 and testing on subsequent stimulation sessions (Day 2 and Day 3). Accuracies were averaged across three independent biological replicates, with each replicate evaluated using five cross-validation folds. Error bars denote the standard deviation across replicates, reflecting variability due to biological and experimental factors. The last row displays the average accuracy per category obtained for the classifier trained on Day 1 and tested on subsequent stimulation sessions by randomizing the neuronal responses for each stimulus, i.e., maintaining the absolute response but shuffling the spatial structure of the spiking activity recorded by the electrodes.}

\label{fig:acc_pretrained}
\end{figure*}


The stimulus amplitude was set to $\SI{4}{\micro\ampere}$ per electrode pair. All digit patterns were presented within the same MEA region, selected for its maximal spontaneous activity and signal quality.
The average classification accuracy per category computed over the three stimulation sessions (Day 1, Day 2, Day 3), and the comparison with the average classification accuracy of the artificial reservoir (AR) computed over different realizations of the noise are summarized in \cref{fig:mean_acc_per_category}.  The mean classification accuracy during each stimulation session across days of stimulation and biological replicates is reported in \cref{tab:acc}. 


\begin{table}[t]
    \centering
    \small
    \renewcommand{\arraystretch}{1.3}
    \setlength{\tabcolsep}{6pt}
    \begin{tabularx}{\linewidth}{l|>{\columncolor{gray!10}}ccc|>{\columncolor{magenta!8}}c}
        \toprule
        \textbf{Stim. day}&\multicolumn{3}{c|}{\textbf{Biological Replicates(\%)}} & \textbf{Mean$\pm$SD(\%)} \\
        \cmidrule(lr){2-4}
        & \textbf{BR 1} & \textbf{BR 2 } & \textbf{BR 3} & \\
        \midrule
        Day 1 & 77 $\pm$ 5 & 67 $\pm$ 9 & 78 $\pm$ 6 & 74 $\pm$ 6 \\
        Day 2 & 78 $\pm$ 5 & 66 $\pm$ 9 & 73 $\pm$ 4 & 72 $\pm$ 6 \\
        Day 3 & 72 $\pm$ 6 & 68 $\pm$ 9 & 67 $\pm$ 4 & 69 $\pm$ 3 \\
        \bottomrule
    \end{tabularx}
    \caption{\textbf{Classification accuracy across stimulation day and biological replicates.} Results are reported for each stimulation session (Day 1, Day 2, Day 3) and for the three biological replicates (BR 1, BR 2, BR 3). Each value indicates the mean classification accuracy and standard deviation across 5-fold validation. The final column shows the average performance across replicates per day.}
    \label{tab:acc}
\end{table}
Interestingly, all biological reservoirs achieved performance levels comparable to those of the artificial reservoir, with an average classification accuracy of approximately 75\%. This consistency was observed across multiple stimulation sessions and among the different biological replicates, underscoring the reliability and reproducibility of the system. Notably, our biological reservoir benchmark capitalizes on the inherent advantages of using a living neural substrate, such as rich, nonlinear dynamics and natural variability, which may offer valuable insights and potential benefits over conventional artificial models.

\subsection{Accuracy Variation Across Days}
In order to assess the stability and generalizability of stimulus-evoked responses over time, we evaluated the classification performance of the classifier trained on data from the first stimulation session and subsequently tested it on data collected in the following days. This cross-day testing approach allows us to probe whether the neural dynamics elicited by a specific set of stimuli remain consistent across days, or if they are subject to spontaneous drift and reorganization.

It is well established that neural cultures evolve dynamically over time, spontaneously transitioning through various activity regimes—from uncoordinated, random spiking to highly synchronized bursting patterns~\cite{fabri, IANNELLO2025116184}. Such spontaneous reorganization is driven by intrinsic developmental processes and changes in connectivity, and it can significantly influence how the network responds to external stimulation. As a consequence, the evoked responses to identical stimulation patterns may vary substantially across days, reflecting underlying shifts in the network’s functional state. 

Then, we used all the neuronal responses to the different stimulus patterns recorded during the first stimulation session (Day 1) to train a linear classifier. The trained model was then evaluated on the data acquired during the subsequent independent stimulation sessions (Day 2 and Day 3), allowing us to assess the temporal stability and generalizability of the biological reservoir's encoding capabilities. The average classification accuracy per category, computed across the three biological replicates, is summarized in \cref{fig:acc_pretrained}. As an additional control, we assessed the classifier's performance on a surrogate dataset in which each neuronal response from the test days was randomized across recording channels. More in detail, we randomized the neuronal responses for each stimulus, maintaining the absolute response but shuffling the spatial structure of the spiking activity recorded by the electrodes. As expected, the classifier failed to discriminate among the stimulus classes under these conditions, yielding a mean accuracy of $12 \pm 5\%$, which is consistent with the chance level expected for a 10-class problem. The results revealed a progressive decrease in classification performance across days, with the accuracy dropping to $46 \pm 15\%$ on Day 2 and further to $37 \pm 19\%$ on Day 3. Although these values remain above chance level (10\%), they indicate a substantial decline in the network's ability to preserve stimulus-specific encoding over time. This performance degradation suggests that the underlying neural dynamics and connectivity patterns within the biological reservoir evolve significantly across days, likely due to spontaneous activity and plasticity phenomena intrinsic to neuronal cultures.

Interestingly, two stimulus categories—specifically, patterns "1" and "7"—consistently maintained higher classification accuracy across all sessions. While the precise reason for this robustness remains unclear, one possible explanation is that these patterns involve a lower number of stimulation electrodes and exhibit minimal spatial overlap with other stimuli. Such properties may lead to more distinct and less noisy evoked responses, facilitating their identification. However, further investigation is required to rigorously assess the relationship between stimulus complexity, spatial interference, and classification stability.
 

